An Efficient Power Management Unit With Continuous MPPT and Energy Recycling for Wireless Millimetric Biomedical Implants

Biomedical implants offer transformative tools to improve medical outcomes. To realize minimally invasive implants with miniaturized volume and weight, wireless power transfer has been extensively studied to replace bulky batteries that dominate the volume of traditional implants and require surgical replacements. Ultra-sonic and magnetoelectric WPT modalities, which leverage low frequency acoustic electrical coupling for energy transduction, become viable solutions for mm-scale receivers. This work presents a fully integrated power management unit for ME WPT in millimetric implants. The PMU achieves load independent maximum power extraction and usage by continuously matching the impedance of the transducer, dynamically optimizing the power stage across varying input divided by load conditions, and reusing the storage energy to sustain the system when input power drops. Its parallel-input regulation and storing stages architecture prevent the cascading power loss. With the skewed-duty-cycle MPPT technique and regulation efficiency optimizer, the PMU achieves a peak MPPT efficiency of 98.5 percent and a peak system overall efficiency of 73.33 percent. Additionally, the PMU includes an adaptive high-voltage charging stage that charges the stimulation capacitor up to 12 V with an improved efficiency of 37.88 percent.

==> table3.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
 &
  \textbf{This Work} &
  \begin{tabular}[c]{@{}c@{}}H.-C Chen,\\ JSSC'21\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}H. Kim,\\ JSSC'21\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}A. Talkhooncheh,\\ JSSC'21\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}J. Li,\\ JSSC'17\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}W. Jung,\\ ISSCC'16\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}X.Yue,\\ ISSCC'23\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}H.-S. Lee,\\ ISSCC'24\end{tabular} \\ \hline
Technology &
  \textbf{180   nm} &
  180   nm &
  180   nm &
  65   nm &
  65   nm &
  180   nm &
  180   nm &
  250   nm \\ \hline
Applications &
  \textbf{\begin{tabular}[c]{@{}c@{}}ME  WPT, \\ implant\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}PV EH, \\ IoT\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}TEG EH, \\ IoT\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}BFC EH, \\ sensor\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}PV EH, \\ IoT\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Battery,\\ IoT\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Piezo EH, \\ IoT\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Inductive, \\ implant\end{tabular} \\ \hline
\multirow{2}{*}{Coverter Topology} &
  \textbf{Buck-Boost} &
  Boost &
  Boost &
  Boost,   Buck &
  Boost,   Buck &
  Buck-Boost &
  Buck-Boost &
  Rectifier \\ \cline{2-9} 
 &
  \textbf{\begin{tabular}[c]{@{}c@{}}Reconfig. \\ SC \\ (12-ratio)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Reconfig. \\ SC \\ (3-ratio)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}CSCR + \\ Reconfig. SC\\ (2/3X,2X)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}Reconfig.  \\ SC  \\ (12-ratio)\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}2,3X   Boost+\\ 6$\sim$9X Boost+\\ 1/4X Buck\end{tabular} &
  \begin{tabular}[c]{@{}c@{}}7b Binary+\\ 2X Boost+\\ 1/3X Buck\end{tabular} &
  Inductive &
  SIMO  R3 \\ \hline
Cascading-Loss Free* &
  \textbf{Y} &
  N &
  N &
  N &
  N &
  N/A &
  N/A &
  Y \\ \hline
\begin{tabular}[c]{@{}c@{}}Fully-Integrated \\ Power Stage\end{tabular} &
  \textbf{Y} &
  Y &
  Y &
  Y &
  Y &
  Y &
  Inductor &
  LC   tank \\ \hline
\begin{tabular}[c]{@{}c@{}}Capacitor \\ Redistribution\end{tabular} &
  \textbf{Y} &
  Y &
  Y &
  N &
  N &
  N &
  N/A &
  N/A \\ \hline
On-chip Cfly &
  \textbf{1.18  nF} &
  2.2  nF &
  10.2  nF &
  N/R &
  0.6   nF &
  3   nF &
  N/A &
  N/A \\ \hline
MPPT Scheme &
  \textbf{Skewed Duty} &
  FOCV &
  SC  PFM &
  2D Hill-Climbing &
  Off-chip &
  N/A &
  Duty  Cycle &
  N/A \\ \hline
Peak ηMPPT &
  \textbf{98.50\%} &
  N/R &
  99.80\% &
  N/R &
  N/R &
  N/A &
  98\% &
  N/A \\ \hline
Vin (V) &
  \textbf{0.7-2} &
  0.45-0.9 &
  0.1-0.5 &
  0.25-1 &
  0.25-0.45 &
  0.9$\sim$4 &
  0$\sim$5 &
  4.8 \\ \hline
Vout (V) &
  \textbf{0-2} &
  1.5 &
  0.75/1.2-1.45 &
  0.9-1.5 &
  3/0.45 &
  0.6/1.2/3.3 &
  0$\sim$5 &
  1-3.5/4.5 \\ \hline
\begin{tabular}[c]{@{}c@{}}Throughput Power \\ (mW)\end{tabular} &
  \textbf{\textless{}3.87***} &
  \textless{}3 &
  \textless{}20.8 &
  \textless{}0.1 &
  \textless{}0.106 &
  \textless{}0.5 &
  N/R &
  135.53 \\ \hline
\begin{tabular}[c]{@{}c@{}}Power/PMU Area** \\ (mW/mm2)\end{tabular} &
  \textbf{3.42} &
  1.77 &
  5.34 &
  0.07 &
  0.22 &
  0.212 &
  N/A &
  N/A \\ \hline
Peak PCE &
  \textbf{\begin{tabular}[c]{@{}c@{}}81.46\%(2/3X)\\ 89.59\%(1X)\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}69.5\%(2X)\\ 65.7\%(1.5X)\end{tabular} &
  85.40\% &
  86\% &
  \begin{tabular}[c]{@{}c@{}}63.8\%\\ (Step-up SC)\end{tabular} &
  81\% &
  N/R &
  90.82\% \\ \hline
Area (mm2) &
  \textbf{1.13} &
  1.69 &
  3.89 &
  1.4 &
  0.48 &
  2.36 &
  0.47 &
  1.56 \\ \hline
\end{tabular}
\end{table*}

==> table_figure.tex <==
\begin{table*}[t]
\begin{center}
\caption{\textbf{Comparisons with State-of-the-Art WPT Technologies for Biomedical Implants}}
\includegraphics[width=7in]{Figure/table.png}
\label{tab1}
\end{center}
\end{table*}
